Towards a General-Purpose Dynamic Information Flow Policy

Noninterference offers a rigorous end-to-end guarantee for secure propagation of information. However, real-world systems almost always involve security requirements that change during program execution, making noninterference inapplicable. Prior works alleviate the limitation to some extent, but even for a veteran in information flow security, understanding the subtleties in the syntax and semantics of each policy is challenging, largely due to very different policy specification languages, and more fundamentally, semantic requirements of each policy. We take a top-down approach and present a novel information flow policy, called Dynamic Release, which allows information flow restrictions to downgrade and upgrade in arbitrary ways. Dynamic Release is formalized on a novel framework that, for the first time, allows us to compare and contrast various dynamic policies in the literature. We show that Dynamic Release generalizes declassification, erasure, delegation and revocation. Moreover, it is the only dynamic policy that is both applicable and correct on a benchmark of tests with dynamic policy.

==> ctable.tex <==
\begin{landscape}

\begin{table*}
\hspace*{-1in}
\begin{tabular}{|l|rrl|}
\hline
\multirow{2}{3cm}{\textbf{Existing Works}} 
& 
\multicolumn{3}{c|}{\textbf{End-to-end Security Definition with policy 
		$\Gamma  $} }
\\ & \multicolumn{3}{c|}{$ \forall c, m, m', \vec{t}, \atke.~~~
\trace = \configs{c, m}\xrightarrow{\vec{t}}{}^* m'  \sat $ }  
\\ \hline
\leftcentering{Static Policy}&   
& $  k_{out}(c, \vec{t}, \atke) ~~~\supseteq $ & 
$\closure{m}_{\eset{\Gamma_{[0]} \LEQ \atke}} $ \\  
\hline
\leftcentering{Delimited Release }&
&$ k_{out}(c, \vec{t}, \atke) ~~~\supseteq $ & 
$ \closure{m}_{(\eset{\Gamma_{[0]} \LEQ \atke} \cup \eset{\Gamma_{[-1]} \LEQ 
\atke})}  
$\\ \hline
\leftcentering{According to Policy} &
$ \forall x \in \Vars. ~\exists F. $ & $
k_{out}(c,\vec{t}, F \AND \atke \AND \{x\}\not \LEQ \atke ) ~~~\supseteq $ & 
$\closure{m}_{\neg \{x\}} $
\\ \hline
\leftcentering{Forgetful Attacker}& 
$ \forall \cod{atk}, i. $  & $
k_{out}(c, \vec{t}_{\pref i}, {F_{\cod{atk}, \atke}}) ~~~\supseteq 
$ & 
$ \closure{m}_{\eset{\Gamma_{[i]} \LEQ \atke}}  ~\cap~k_{out}(c, \vec{t}_{\pref 
i-1}, 
{F_{\cod{atk}, \atke}})  $ \\\hline
\leftcentering{Paralock}&
$ \forall A, i.$ & $
\cod{unlock}(\trace_{[i]}) \subseteq \vec{k}_A \sat~ 
k_{out}(c, \vec{t}_{\pref i},  A) ~~~~\supseteq $  
& $ \closure{m}_{\eset{A}} \cap k_{out}(c, \vec{t}_{\pref i-1}, A) $ \\ \hline
%\leftcentering{Paralock original}&
%$ \forall A, i.$ & $
%\cod{unlock}(\trace_{[i]}) \subseteq \vec{k}_A \sat~ 
%k_{2}(c, \vec{t}_{\pref i},  A) ~~~~= $  
%& $ k_{2}(c, \vec{t}_{\pref i-1},  A)  $ \\ \hline
\leftcentering{Crypto}&
$ \forall i, j, n.$ & $
k_4(c, \atke, \vec{t}_{[i,n]}) ~~~\supseteq $ &
$\bigcap_{i\leq j \leq n}\closure{m}_{\eset{\Gamma_{[j]} \LEQ \atke}} $ \\\hline
%\leftcentering{Non-Static Policy}& 
%$ \forall e \in \Objs, i. $ & 
%$k_{out}(c,\vec{t}_{\pref i}, \atke \AND \{e\} \not 
%\LEQ \atke) ~~~\supseteq$ & 
%$ [m]_{\neg \{e\}} \cap \cod{MemK}(c,m,i, \atke) $
%\\\hline
\leftcentering{Non-Static Policy}& 
$ \forall i. $ & 
$k_{out}(c,\vec{t}_{\pref i}, \atke \AND \eset{ \Gamma_{[i]} \not \LEQ a}\not 
\LEQ \atke) ~~~\supseteq$ & 
$ \closure{m}_{\eset{\Gamma_{[i]} \LEQ a}} \cap \cod{MemK}(c,m,i, \atke) $
\\\hline
\end{tabular}
\caption{End-to-End Security Property in Existing Works.}
\label{tab:summary}
\end{table*}

\begin{table*}
\hspace*{-1in}
\begin{tabular}{|l||C{1cm}C{1cm}|C{1cm}C{1cm}|C{1cm}C{1cm}|C{1cm}C{1cm}||c|c|}
	\hline
 & \multicolumn{2}{C{2cm}|}{\centercentering{Declassification}} 
 & \multicolumn{2}{C{2cm}|}{\centercentering{Erasure}} 
 & \multicolumn{2}{C{2cm}|}{\centercentering{Revocation}}
 & \multicolumn{2}{C{2cm}||}{\centercentering{Miscellany}} 
 &&\\ \cline{2-9}
 & Accept &Reject & Accept & Reject &Accept & Reject  &Accept & Reject  
 & SemCon & Landry \\
& Sec & InSec & Sec & InSec & Sec & InSec & Sec & InSec && \\ \hline
Static Policy &\no&\yes&\yes&\no&\yes&\no &\no&\no && \\	
Delimited Release &\yes&\no&\yes&\no&\yes&\no &\yes&\no && \\	
According to Policy &\yes &\yes&\yes &\yes&\no&\yes &\no&\yes && \\	
Forgetful Attacker &\yes&\yes&\yes&\yes&\yes&\yes &\yes&\yes && \\	
Paralock &\yes&\yes&\wrong&\no&\wrong&\yes &\wrong&\no && \\	
Crypto &\yes&\wrong&\yes&\wrong&\no&\wrong &\no&\wrong && \\ 
%Piecewise &\yes &\yes &\yes &? &\no &  ?& &  && \\ 
%\hline	
%According + Paralock &\yes &\yes &\yes & \yes & \wrong &  \yes& \wrong & \yes 
%&& \\ 
\hline
Non-Static Policy &\yes&\yes&\yes&\yes&\yes&\yes &\yes&\yes && \\	\hline
\end{tabular}
\caption{Property of Existing End-to-End Guarantees. 
\\ \yes: ~provided guarantee is applicable and consistent.
\\ \no: ~inconsistent and not intended 
\\ \wrong: ~inconsistent but intended}
\label{tab:property}
\end{table*}

\end{landscape}


==> erasure.tex <==
\begin{figure}
	\begin{mathpar}
%		\zero(\Mt,\eta, x)(v) = 
%		\begin{cases}
%			0, &  x \in \free(v) \\
%			\Mt(v), & \text{otherwise}
%		\end{cases} 
%		 \\
		\switch(\Mt, x, \eta)(\varx) =
		\begin{cases}
			0, &\! x \in \free(\varx) ∧ x'\not\in \liveset{\actset'}(\eta)\\ %\AND \labelof{\varx}{\Mt} \absleq L \\
			%[0], & x \in \free(\varx) \AND \labelof{\varx}{\Mt} \not \absleq L  \\
			\Mt(\varx), &\! \text{otherwise}\\
		\end{cases}
	\end{mathpar}
	\[	
	\inferrule*[right=ST-Erase]
	{ \configTwo{\Mt}{x} \evalto n 
			\quad \Mt' = \Mt\Mupdate{x}{n}}
	{ \configTwo{\Mt}{\assigneta{x}{e}}\ERTo{\actset'} \configTwo{\switch(\Mt', x)}{\Skip}}	\\
	\]
%	\[ 
%	\inferrule*[right=ST-Phi-Switch]
%	{ X = \difffunc(\actset_1,\actset_2) 
%		\quad \Mt' = \Mt\Mupdate{\overrightarrow{\actset_1(X)}}{\overrightarrow{\actset_2(X)}} }
%	{ \configTwo{\Mt}{\phiassigneta{\actset_1}{\actset_2}}\To \configTwo{\switch(\Mt', \overrightarrow{\actset_1(X)})}{\Skip}}	
%	\]
	\caption{Erasure Semantics of Assignment.}
        \label{fig:erasure}	
\end{figure}


%\begin{figure}
%	\begin{mathpar}
%		\inferrule[S-Asgn1-E] 
%		{\configTwo{\Mt}{e} \evalto {n} \\ \labelof{x}{\Mt}\sqsubseteq L \quad \Mt' = \switch(\Mt\Mupdate{x}{n}, \eta)}
%		{\configTwo{\Mt}{\assigneta{x}{e}} \To  \configTwo{\Mt'}{\Skip}}	
%		\and 
%		\inferrule[S-Asgn2-E] 
%		{\configTwo{\Mt}{e} \evalto {n} \\ \labelof{x}{\Mt}\not\sqsubseteq L \quad \Mt' = \switch(\Mt\Mupdate{x}{[n]}, \eta)}
%		{\configTwo{\Mt}{\assigneta{x}{e}} \To \configTwo{\Mt'}{\Skip}}	
%		\and
%		\inferrule[S-Asgn3-E] 
%		{\configTwo{\Mt}{e} \evalto {[n]} \quad \Mt' = \switch(\Mt\Mupdate{x}{[n]}, \eta)}
%		{\configTwo{\Mt}{\assigneta{x}{e}} \To  \configTwo{\Mt'}{\Skip}}	
%		\and 	
%	\end{mathpar}
%	\caption{Erasure Semantics}
%	\label{figure:erasure}
%\end{figure}


==> label-encoding.tex <==


\subsection{Encoding Existing Security Specifications}
\label{sec:encoding}
We show next that our dynamic policy specificatin is (1) expressive enough
to encode existing policies, and (2) bridges current gaps between various
policy specifications.

Before diving into a particular policy, we first note that as shown in
Section~\ref{sec:background}, there are two major approaches of specifying
sensitivity change:
\begin{itemize}
\item Mutable Denning-Style Label:
The first approach is to change the security level from $\ell_1$ to $\ell_2$,
where both $\ell_1$ and $\ell_2$ are drawn from a Denning-style lattice $
\Lattice $. To encode such mutable Denning-Style label, we can define
corresponding level sets  $L_1$ to $L_2$ as follows:
\begin{equation}
\label{eq:denning}
\AllLevels = \{\ell ~|~ \ell\in \Lattice \};~\forall i\in\{1,2\}.~L_i \defn 
\{\ell' 
~|~\ell_i \LEQ \ell' \}
\end{equation}
Hence, a change from $\ell_1$ to $\ell_2$ can be encoded as a change from $L_1$
to $L_2$.

\item Mutable Lattice: the second approach is to change the partial ordering on
security levels~\cite{Arden:2015csf, rolebased, myers2000}, where security
levels are principals such as $ \cod{Alice}, \cod{Bob}, \cod{John} $. In this
approach, principals form a lattice according to the acts-for relationship:
$P_1\sqsubseteq P_2 \Leftrightarrow  P_2~\cod{actsfor}~P_1$. Unlike the first 
approach,
information is always associated with a fixed principal. However, the acts-for
relationship can be granted or revoked during program execution.

To encode a mutable lattice, we explicitly interpret each principal $P$ as a
set of principals who \emph{currently} acts for $P$. Hence, when the acts-for
relation changes from $\cod{actsfor}_1$ to $\cod{actsfor}_2$, $L_1$ and $L_2$
below encodes $P\in \mathbb{P}$ before and after the change respectively:
\begin{equation}
\label{eq:principalbased}
\AllLevels = \mathcal{P}(\mathbb{P});~\forall i\in\{1,2\}.~L_i \defn \{P'\in 
\mathbb{P}
~|~P'~\cod{actsfor}_i~P \}
\end{equation}
Hence, the change from from $\cod{actsfor}_1$ to $\cod{actsfor}_2$ can be
encoded as a change from $L_1$ to $L_2$.
\end{itemize}

Next, we show at how to encode existing security specifications into our
language in~\ref{fig:while-syntax} and informally adjust the encodings; the
faithfulness of encodings is proved in Section~\ref{sec:semantics}.

\subsubsection{Delimited Release}
\label{sec:hatch}

Delimited Release~\cite{sabelfeld2003} uses \emph{Escape Hatches} to
support declassification. An escape hatch has the form of $ \cod{declassify}(e,
\ell) $, which downgrades the sensitivity of $ e $ to level $ \ell $ drawn from
a Denning-style lattice. Delimited Release requires a programer to explicitly
insert \emph{escape hatch} into the source code to allow declassification.

As stated in~\cite{sabelfeld2003}, ``all of the declassified expressions
are assumed to be released'' in the delimited release policy. For example, a
hatch $ \cod{declassify}(e, \ell) $ downgrades the policy on $e$ even if the
hatch is never executed (i.e., dead code). Hence, we can encode Delimited
Release as:
\[
\spec(\sentity)=L_{\Gamma(\sentity)}\cup \bigcup_{\cod{declassify}(\sentity, 
\ell)} L_\ell
\]
where  $L_\ell$ is the encoding of $\ell$ according to
Equation~(\ref{eq:denning}).

\if0
To encode each escape hatch $ \cod{declassify}(e_i, \ell_i) $, we first convert
the level $ \ell_i $ to $ L_i $ as in Equation~(\ref{eq:denning}) and introduce
a distinguished security event $ s_i $ for the $i$-th escape hatch, and replace
the $i$-th escape hatch command in the program $ \cod{declassify}(e_i, \ell_i)
$ with $\cod{EventOn}(s_i)  $. 
The expression $ e $ in $ \cod{declassify}(e_i, \ell_i) $ is labeled as:
 \[ \spec(e)= s_i?L_i \leftarrow  L_{i-1} \]
where $L_{i-1}$ is the sensitivity of $e_i$ right before the escape hatch or 
the initial sensitivity $ L_0 $ at the beginning of the program. In case an 
expression $e$ is declassified in multiple hatches, i.e., there is a
series of hatches: $ \cod{declassify}(e, \ell_1);...; \cod{declassify}(e,
\ell_n) $, where $ \ell_n \LEQ ... \LEQ \ell_1 $(no upgrading), we utilize the
nested dynamic policy specification:
\[
\spec(e)= s_1?...(s_n?L_n\leftarrow L_{n-1})...\leftarrow  L_0
\]
\fi
%Consider the average salary example shown in their paper, 
%where $ h_1, ..., h_n $ initially store the salaries of $ n $ employees. 
%The average of their salary 
%is intentionally released, while the precise salary of each individual is kept 
%secret. Such a policy can be specified as the following escapes hatch:
%
%\begin{lstlisting}[numbers=none, xleftmargin=25pt]
%$ avg = \cod{declassify}((h_1+ · · · + h_n)/n, L); $
%\end{lstlisting} 
%
%Following the encoding approach, we associate the expression $ (h_1+... + 
%h_n)/n $ with security label $ s_{avg}?L\leftarrow H $: 
%\[
%\spec((h_1+... + h_n)/n) = s_{avg}?L\leftarrow H
%\] 
%and replace the escape hatch with:
%\begin{align*}
%&\cod{EventOn}(s_{avg});\\
%&avg = (h_1+ · · · + h_n)/n; 
%\end{align*} 
\subsubsection{Gradual Release~\cite{askarov2007}}
\label{sec:GRsyntax}
%First, we provide the encoding of a release event.
In Gradual Release, a release event is generated by a special command $
x:=\cod{declassify}(e) $ which releases the value of $ e $ to the memory
channel of label $\spec(x)$. Informally, a gradual release policy is satisfied
when information leaksage only occurs with release events. Hence, we encode a
release event as
\[\cod{EventOn}(r);x:=e;\outcmd{\Gamma(x)}{e};\cod{EventOff}(r);\] where $r$ is
a distinguished event for release, and we set
$\forall e. ~\Gamma'(e)=r?\mathbb{L}\leftrightarrows\Gamma(e)$ to state that 
leaksage is
allowed when there is a release event, but otherwise, the information flow
restriction of $\Gamma$ is obeyed.

\ifscopedsecrets
\subsubsection{Scoped Secrets}
Hunt and Sands~\cite{hunt2008} propose a
special command to support erasure policy, in the form of 
%
\[ \cod{input}~x: \ell_1 \nearrow \ell_2 ~\cod{in}~ C \] 
%
where the input $x$ has security level $\ell_1$ in $C$, but it will be erased
to level $\ell_2$ after $C$ finishes execution; $\ell_1, \ell_2$ are drawn from
a Denning-style lattice. 

To encode the special command, we replace it with:
\[
C; \cod{EventOn}(s_x)
\]
where  $ s_x $ is a unique event for the code block. Then, the dynamic
policy on $x$ is specified as:\footnote{Since the $\cod{input}$ statement
in~\cite{hunt2008} assumes no duplicated input variable names, there is no
need of nested policies.}
\[ \spec(x)=s_x? L_2 \leftarrow L_1  \]
where $L_1, L_2$ are the encodings of $\ell_1, \ell_2$ respectively 
according to the conversion in
Equation~(\ref{eq:denning}).
\fi

\subsubsection{Compound Label}\label{sec:complabel}

A few security policies~\cite{chong2005,chong2008,askarov2015} use
a similar security specification despite various scopes and end-to-end security
definitions. We call such specification \emph{compound label} as it is either a
simple level $ \ell $ drawn from a Denning-style lattice, or in the form of $
q_1 \abv{e}{\rightarrow}  q_2 $, where $q_1$ and $q_2$ are themselves compound
labels.  Informally, $ q_1 \abv{e}{\rightarrow} q_2 $ specifies that the
sensitivity changes from $ q_1 $ to $ q_2 $ once the condition $ e $ is
satisfied. For example, a label $ (\High \abv{e_1}{\rightarrow}\Low)
\abv{e_2}{\rightarrow} \High $ specifies that the sensitivity first downgrades
from $ \High $ to $ \Low $ when expression $ e_1 $ is satisfied. Then, 
sensitivity is upgraded (erased) to $ \High $ when expression $ e_2 $ is
satisfied.
% All according to policy labels are
% global, i.e., they govern all source code in scope. Hence, no policy command 
%is
% inserted to the source code. 

Let $L_{\ell}$ be the encoding of a level $ \ell $ in a Denning-style lattice
according to Equation~(\ref{eq:denning}). Then we can define a conversion
function $\cod{cvt}$ for a compound label as follows:
\begin{align*}
\cod{cvt}(\ell) &= L_{\ell}\\
\cod{cvt}(q_1  \abv{e}{\rightarrow} q_2) &= 
e?\cod{cvt}(q_2)\leftarrow \cod{cvt}(q_1)
\end{align*}

\if0
\subsubsection{Principal-Based Labels}
\label{sec:principal}
Principal-based labels~\cite{Arden:2015csf, JRIF,Broberg:2010popl} use
principals, such as $ Alice, Bob, John $ as the basic entity of sensitivity.
Similar to labels drawn from an immutable lattice, the acts-for relationship,
denoted as $ \actsfor $, defines the relation on principals. For example, a
principal $ Alice $ may access information of $ Bob $ iff $ Alice \actsfor Bob
$ (Alice acts for Bob). However, dynamic policy based on principals are
different in two aspects:
\begin{itemize}
\item  The security entities in a principal-based model are associated with
\emph{immutable} principals, representing ownership. However, the security
entities in a label-based model have \emph{mutable} labels.

\item To enable dynamic policy, the acts-for relation, therefore the lattice
on principals, can change dynamically. The changes are typically specified by
special commands such as $ \cod{actsfor} $ and $ \cod{revoke} $.  However,
label-based model assumes an \emph{immutable} lattice of levels.
\end{itemize}

%Going back to the two scenarios we presented before. The first scenario, 
%where a variable $ x $ downgrades from $ H $ to $ L $, is easily encoded by 
%our formalization as below, where $ \gamma $ is before downgrading and $ 
%\gamma' $ is after. 
%\begin{align*}
%\gamma(x) &= H;\\
%\gamma'(x) &= L;
%\end{align*} 

For example, consider information labeled as $ Alice $ with no acts-for
relation initially. Bob is unable to access the information since he does not
act for Alice. Bob is allowed to access the information only when it is
downgraded at certain point, with $ Bob \actsfor Alice $ enable by policy.

To encode principal-based models, we explicitly interpret each label $p$ as a
set of principals who acts for $p$ at each program point. For example, before
the downgrading, we have 
\[ \cod{Alice} \mapsto \{Alice\} \text{ and } \cod{Bob} \mapsto \{Bob\} \]
Once $ Bob \actsfor Alice $, we have 
\[  \cod{Alice} \mapsto \{Alice, Bob\} \text{ and } \cod{Bob} \mapsto \{Bob\}
\]

We use security event $ s_{p_1 \actsfor p_2} $ to record the acts-for relation
of $ p_1 \actsfor p_2 $. The event is set to $\True$ when $ p_1 $ acts for $
p_2$, and $\False$ when the relation is revoked or absent. We define $
\cod{Acts}(p, \secm) $ to extract all the principals that the principal $ P $
current acts for recorded in the execution memory $ m $:
\[
\cod{Acts}(p, \secm) = \{p_1 ~|~\forall p_1 \in \mathbf{P}.~ \secm(s_{p 
\actsfor p_1}) \OR p_1 = p\}
\]

To define the interpretation function, we define $ \cod{ACT}(\pr, \sevent) $
that takes in a principal $ \pr $ and a series of security events $ \sevent $,
and returns the set of the principals who \emph{directly} acts-for $\pr$:
\begin{multline*}
\cod{ACT}(\pr, \sevent) = \{\pr' ~|~\exists i~.~s[i] = 
\cod{actsfor}(\pr', \pr) \\ \AND \cod{revoke}(\pr', \pr)\not\in  
\sevent_{\succcurlyeq i} \}
\end{multline*}

\alglanguage{pseudocode}
\begin{algorithm}
	\caption{Breadth-First Search for Acts-for Principals}
	\label{alg:search}
	\begin{algorithmic}[1]
		\Function{BFSAct}{$\pr, \vec{s}$}
		\State 	$ worklist \gets [\pr]$ \Comment FIFS Queue
		\State 	$ aset \gets \{\pr \} $ \Comment Set with unique items 
		\While {$worklist \not = \emptyset $} 
		\State $ item \gets worklist.pop() $
		\State $ worklist.append(ACT(item, \vec{s})-aset)  $ \Comment set 
		subtraction
		\State $ aset.add(ACT(item, \vec{s}))  $
		
		\EndWhile
		\State \Return $ aset $
		\EndFunction
	\end{algorithmic}
\end{algorithm}

Note that with a sequence of security events $\sevent$, the direct acts-for
relationship induces a relation $R_{\sevent}$ on principals: $\pr_1~R~\pr_2$
iff $\pr_2 \in \cod{ACT}(\pr_1, \sevent)$. Hence, we can compute the
\emph{transitive closure} of $R_{\sevent}$, denoted by $R_{\sevent}^+$, which
is exactly the set of principals who can access data tagged with $\pr$:
%corded by $ \cod{ACT} $ function, we can compute all
%the principals that currently acts-for using a simple search algorithm as shown
%in Algorithm~\ref{alg:search}. The label interpretation function is defined as 
%below:
\[
\intfun(\pr, \sevent) = R_{\sevent}^+(\pr)
\]

The sensitivity of a principal $ p $ is set of principals that  $ p $ 
current acts-for and $ p $ itself. Thus, the security labels for each principal 
$ p \in \mathbf{P} $ using security 
event \DZ{the definition does not handle transitivity}:
\[
 \{p\} \join \Big( \bigsqcup_{\forall p_1 \in \mathbf{P}}{s_{p\actsfor 
p_1}?\{p_1\}\leftrightarrow\emptyset} \Big) 
\]
\fi

%\subsubsection{Flow Locks and Paralocks}
%\label{sec:paralock-label}
%Flow Locks~\cite{Broberg:2006esop} and its successor
%Paralocks~\cite{Broberg:2010popl} introduce \emph{locks}, denoted as $ \lock $ 
%to enable dynamic policy.  Let ${\lockset}$ be a set of locks, and 
%$\mathbb{P}$ be a set of
%principals.  A Paralock policy is specified with the following components:
%\begin{itemize}
%\item Flow locks in the form of $\lockset \sat P$ where $ \lockset \subseteq 
%\alllocks$ is the 
%lock set for principal $ P\in \mathbb{P}$.
%
%\item Distinguished commands $\cod{open}(\lock), \cod{close}(\lock)$ that 
%open and close the lock  $\lock \in \alllocks$.
%\end{itemize}
%
%To simplify notation, we use $ \spec(x, P) = \lockset $ to denote the fact that
%$ \{\lockset \sat P\}$ is part of the security policy of $ x $, otherwise $
%\spec(x, P) = \top $. Paralocks security is formalized as \emph{an extension}
%of gradual release. In particular, Paralock security is defined based on
%\emph{sub-security condition} for each hypothetical attacker 
%$A=(P_A,\lockset_A)$
%where $P_A\in \mathbb{P}$ and $\lockset_A\subseteq \alllocks$:
%\begin{itemize}
%\item A variable is considered ``public'' for attacker $A$ when $ \spec(x, P_A)
%= \lockset_x \subseteq \lockset_A$; otherwise, considered ``secret''.
%
%\item A ``release event'', in gradual release sense, is defined as a period of
%program execution when the set of \emph{opened} locks $\lockset_{open} 
%\subseteq
%\lockset_A$.
%\end{itemize}
%
%Hence, for each concrete $A=(P_A,\lockset_A)$, we can encode Paralock security
%as follows:
%\begin{itemize}
%\item  We define a security event $ s_{\lock} $ for each lock $ \lock \in 
%\lockset $
%and the lock command $ \cod{open}(\lock) $ (resp. $ \cod{close}(\lock) $) is 
%converted
%to $ \cod{EventOn}(s_\lock) $ (resp. $ \cod{EventOff}(s_\lock))$.
%
%\item Let $\Gamma(x)=\{P_A\}$ when $ \spec(x, P_A) = \lockset_x \subseteq
%\lockset_A$; otherwise, $\Gamma(x)=\{\} $ (i.e., secret for $P_A$).  
%
%\item Following the encoding of gradual release, we define
%$\Gamma'(x)=cnd?\Gamma(x):\{P_A\}$ where $cnd \defn \neg \bigwedge_{\lock \not 
%\in \lockset_A} s_\lock$, i.e., all locks not in $\lockset_A$ must be 
%currently 
%closed, which implies an output event (not a release event):  
%$\lockset_{open} \subseteq \lockset_A$; otherwise, for a release event, $ x $ 
%is public to $ P_A $.
%\end{itemize}
%
%\input{paralocktrans}
%As a concrete example, we show the original Paralock code and its transform
%code in Figure~\ref{fig:paraloctrans} for $A=\configs{a,\{D\}}$. We note that
%under the encoding, the first assignment $y:=x$ is under a release event since
%only lock $D$ is open, which is a subset of $\lockset_A=\{D\}$; both the output
%channel and the value can be read by $a$. On the other hand, the second
%assignment $z:=y$ is \emph{not} under a release event, as a opened lock $N$ is
%not possessed by attacker $A$. This is also reflected by the encoding: while
%the output channel is observable to $a$ unconditionally, the value of $y$ has
%policy $\{\}$ at that point, as $s_N=\True$.
%
%Hence, we can encode Paralock policy by explicitly checking each transformed
%program under gradual release policy for each $A$, and accept the program iff
%all transformed programs are secure.

\ifforgetful
\subsection{Forgetful Attacker} 
\DZ{Do we need to introduce forgetful attacker model?}
\fi

\if0 REMOVED FOR NOW
\subsubsection{JRIF}
Kozyri et al.~\cite{JRIF} use an automaton for each
variable to specify a dynamic policy. An automaton $ \autom$ is defined as
$\configs{Q, \Sigma, \delta, q_0, Prins} $ where $ Q $ is set of states, $
\Sigma= \{F_1, ..., F_n\} $ is set of $ \cod{classifier}  $, $ \delta: Q \times 
\Sigma \mapsto Q $ is a total, deterministic
the transition function, $ q_0 $ is the initial state, and $ Princs $ is a
mapping from states to sensitivity levels in a security lattice. 
The mutation of sensitivity is triggered by manually inserted statement $ 
\cod{reclassify}(e, F) $.   For example,
Figure~\ref{fig:example:jrif} (adapted from Figure 2 in \cite{JRIF})
presents a simple JRIF automaton with two states $ Q = \{ q_0, q_1 \} $ and
two classifiers $ \Sigma = \{ \cod{noti},\neg\cod{noti} \}$. The $ 
Princes $ maps the the starting state $ q_0 $ to $ H $ and $ q_1 $ to $ L $.  
. This automaton models the reviews
score is initially secrete(H) to the authors, later when the notification date
arrives (trigged by an inserted command $ \cod{reclassify}(review, \cod{noti}) $
in the program), the review score is declassified to L.
\begin{figure}
	\centering
	\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto] 
	\node[state,initial] (q_0)   {$q_0 (H)$}; 
	\node[state] (q_1) [right=of q_0] {$q_1(L)$}; 
	%   \node[state] (q_2) [below right=of q_0] {$r$}; 
	\path[->] 
	(q_0) edge [loop above] node {$ \neg \cod{noti} $} ()
	edge  node {$ \cod{noti} $} (q_1)
	%          edge  node [swap] {$ \cod{log} $} (q_2)
	(q_1) edge [loop above] node {*} ();
	%    (q_2) edge [loop right] node {*} ();
	\end{tikzpicture}
	\caption{Example: JRIF Automaton}
	\label{fig:example:jrif}
\end{figure}

\DZ{Where is the encoding?}
\fi

%JRIF uses an explicit command $
%\cod{reclassify(e, F)} $ as dynamic modifier to change the sensitivity, where 
%$ 
%e $ is an expression and $ F $ is an classifier.  
%The security evaluation rule for the $ \cod{reclassify}(e,F) $ 
%expression looks like below that the $ \vec{F} $ are all the seen classifiers 
%of the trace: 
%\[ \configs{\cod{reclassify}(e,F), m} \xrightarrow[F]{}  \configs{e, m} \]
%
%We define the evaluation function of the automaton $\configs{Q, \Sigma, 
%\delta, 
%q_0, Prins} $  given a series of classifiers $ \configs{F_1, F_2, 
%..., F_n} $ as 
%\begin{align*}
%\cod{aut}(\autom, \varepsilon) & = q_0\\
%\cod{aut}(\autom, \configs{F_1, F_2, ..., F_n}) &= \delta(\cod{aut}(\autom, 
%\configs{F_1, F_2, 	..., F_n}
%\end{align*}
%%The policy event in this policy is the classifiers emitted during the 
%%statements $ \vec{\pevent} = \configs{F_1, F_2, ..., F_n} $. This policy is 
%%also an $ \ipolicy $:
%%\[ \ipolicy(x, \tau) = \cod{aut}(\tagfun(x), \vec{\pevent}) \]
%
%Using the syntax of our formalization, we have:
%\begin{align*}
%&&& &x: \\
%& \cod{reclassify}(e,F) &\hookrightarrow& 
%& \cod{Event}(F)
%\end{align*}


==> proof.tex <==
%\textbf{Proofs for Equivalent Formalizations}


%
%\noindent\textbf{\textit{Lemma~\ref{lemma:static-eq}.} }
%With $\sim \defn \sim_{\cod{NI}}$ and 
%$\allowence \defn \allowence_{\cod{NI}}$,
%Definition~\ref{def:framework} is equivalent to
%the knowledge-based noninterference definition:
%\begin{multline*}
%\forall c, m, l, i, \vec{t}.~ \configs{c,m} \termout \vec{t} \implies \\
%k(c,m,\vec{t}_{[:i]},\Gamma)=\closure{m}_{l, \Gamma}  \iff 
%\mathcal{K}(c,\vec{t}_{[:i]}, \sim_{\cod{NI}})\supseteq
%\closure{m}_{l,\Gamma}
%\end{multline*}
%\begin{proof} 
%This is a direct implication of Lemma~\ref{lem:convert} when 
%\[ M: = \closure{m}_{l, \Gamma}, ~~~~\vec{t} := \vec{t}_{[:i]}\]
%We have $\closure{m}_{l, \Gamma} 
%\subseteq \closure{m}_{l, 
%\Gamma} $ trivially, and  $ k(c,m,\vec{t}_{[:i]},\Gamma) \subseteq 
%\closure{m}_{l, \Gamma}$ from the monotonicity of the knowledge.
%\end{proof}
%

%
%\noindent\textbf{\textit{Lemma~\ref{lemma:delimited-eq}.} }
%With $\sim \defn \sim_{\cod{NI}}$ and $\allowence \defn 
%\closure{m}_{l,\Gamma'}  
%$,
%Definition~\ref{def:framework} is equivalent to Definition~\ref{def:delimited}.
%\begin{proof} First, we convert a security levels $ \ell $ from the Denning's 
%style to our attacker levels $ l $ as described in Section~\ref{sec:syntax},  
%and outputs the terminating memory of the trace to its variable's level. That 
%is,
%\begin{multline*}
%\forall c, m, m', \sentity, \Gamma. \configs{c, m} \rightarrow^* m'  \iff 
%\configs{c, m} \termout \vec{t}  \\
%\AND \vec{t} = \configs{ \configs{ch, n, 
%\gamma}~|~ ch = \sentity \AND n = m'(\sentity) \AND \gamma = \Gamma } 
%\end{multline*}
%Thus, we rewrite Definition~\ref{def:delimited} in following two-run style:
%\begin{multline*}
%\forall c, m_1, m_2, l.\\
%m_1 \loweq_{l}^{\Gamma'} m_2 \AND \configs{c, m_1}\termout \vec{t}   
%\AND \configs{c, m_2} \termout \vec{t}_2 \\
%\sat \proj{\vec{t}_1}_{l} = \proj{\vec{t}_2}_{l} 
%\end{multline*}
%The proof then follows the equivalence proof of knowledge-based and two-run
%style noninterference definition~ (Lemma~\ref{lemma:static-eq}). 
%%Note that
%%Definition~\ref{def:delimited} assumes program termination and one observation
%%at the end of program execution. Hence, the equivalence relation $\pref$ can
%%also be replaced with equality or postfix.
%\end{proof}




\noindent\textbf{\textit{Lemma.}} Paralock's policy on 
each Attacker $ A = (a, \lockset_A) $ is equivalent to a Gradual Release policy 
with:\\
(1) $ \Gamma_A $, that $ \forall x \in \Vars. \Gamma_A(x) = \spec(x, a) $, and 
\\
(2) speciflized semantics $ \dashrightarrow_A $:
\begin{mathpar}
	\inferrule[Output Event]{ \configs{e,m}\evalto n 
		\and l = \configs{x, n, \lockset} 
		\and \lockset \subseteq \lockset_A}
	{\configs{x:=e,m,\lockset} \dashrightarrow^{l}_A \configs{\Skip, 
			m,\lockset}}
	\and
	\inferrule[Release Output Event]{ \configs{e,m}\evalto n 
		\and r = \configs{x, n, \lockset}
		\and \lockset \not  \subseteq \lockset_A}
	{\configs{x:=e,m,\lockset} \dashrightarrow^{r}_A \configs{\Skip, 
			m,\lockset}}
\end{mathpar}
For simplicity, we use the following language, where $ c $ is supported in both 
original papers. 
\begin{align*}
c ~::=~& \Skip~|~x:=e~|~c_1;c_2~|~\ifcmd{e}{c_1}{c_2}~\\
& |~\while{e}{c}\\
c^{\cod{GR}} ~::=~& c~|~x:=\declassify(e)\\
c^{\cod{PL}} ~::=~& c~|~\cod{open}(\lockset) ~|~ \cod{close}(\lockset), 
~~\lockset \in \mathbf{Locks}
\end{align*}
Paralock uses $ \lockset $ to track the current open locks in the semantics. 
$ \lockset_1 + \lockset_2 $ takes a union of the two lock sets, while $ 
\lockset_1 - \lockset_2 $ removes from $ \lockset_1 $ any lock that also exists 
in $ \lockset_2 $.
\begin{mathpar}
\inferrule{}{\configs{\cod{open}(\lockset_1),m,\lockset} \To \configs{\Skip, m, 
\lockset + \lockset_1}}
\and
\inferrule{}{\configs{\cod{close}(\lockset_1),m,\lockset} \To \configs{\Skip, 
m, \lockset - \lockset_1}}
\and
\inferrule{ 
\configs{e,m}\evalto n \and t = \configs{x, n, \lockset}}
{\configs{x:=e,m,\lockset} \xrightarrow{t} \configs{\Skip, 
		m[x\mapsto n],\lockset}}
\end{mathpar}
In Paralock, an attacker is modeled as $ A = (a, \lockset_A) $. 
For an output event $ t= \configs{x, n, \lockset} $, it is visible to the 
attacker if the attacker have 
all the locks required by the output channel $ x $:  $  \spec(x, a) \subseteq 
\lockset_A $. So, the $ A $-visible part of output sequence $ \vec{t} $, 
denoted as $ \proj{\vec{t}}_A $, is:
\begin{multline*}
\proj{t}_A \defn \configs{\configs{x,n,\lockset}~|~ \forall 
\configs{x,n,\lockset} \in 
\vec{t}. ~A = (a, \lockset_A)
\\ \AND  \spec(x, a) \subseteq \lockset_A } 
\end{multline*}
Two memory $ m_1, m_2 $ look the same to attacker $ A $ if the visible part of 
the memory is the same:
\begin{multline*}
\forall a, \lockset_A, A, m_1, m_2.~\\
m_1 \loweq_{A} m_2  \AND A = (a, \lockset_A) 
\iff \\
\forall x \in \Vars. ~\spec(x, a)  \subseteq 
\lockset_A \sat m_1(x) = m_2(x)
\end{multline*}
The attacker's knowledge in Paralock is defined as follow:
\begin{multline*}
k_{\cod{PL}}(c,m,\vec{t}, A) = \{ m' ~|~ m \loweq_{A} m' \\
\AND  \configs{c, m', \lockset} \xrightarrow{\vec{t_1}} \configs{c',m'', 
	\lockset'} \xrightarrow{\vec{t_2}} m'''  \AND \proj{\vec{t_1}}_A = 
\proj{\vec{t}}_A
\}
\end{multline*}

\begin{Definition}[Paralock Security]
\begin{multline*}
\forall c, m, m', \lockset, \vec{t}, a, \lockset_A, A, i. \\
\configs{c,m, \lockset} \xrightarrow{\vec{t}}m' \AND  A = (a, \lockset_A) \AND  
\\
\vec{t}_{[i]}.\lockset  \subseteq \lockset_A \implies
k_{\cod{PL}}(c,m,\vec{t}_{[:i]}, A) = k_{\cod{PL}}(c,m,\vec{t}_{[:i-1]}, A)
\end{multline*}
\end{Definition}
The semantics of Gradual Release are shown as below:
\begin{mathpar}
\inferrule[Output Event]{\configs{e,m}\evalto n \and l = \configs{x, n}}
{\configs{x:=e,m} \xrightarrow{l} \configs{\Skip, m[x\mapsto n]}}
\and
\inferrule[Release Output Event]{\configs{e,m}\evalto n \and r = \configs{x, 
n}}
{\configs{x:=\declassify(e),m} \xrightarrow{r} 
\configs{\Skip, m[x\mapsto n]}}
\end{mathpar}

In Gradual Release,
an attacker is modeled as a level $  \ell \in  \Lattice $ in a Denning's 
Lattice, and $ \Gamma $ specifies the visibility of the attacker. For an 
event $ t=\configs{x, n} $ (either $ l $ or $ r $), it is visible to the 
attacker if $ \Gamma(x) \LEQ \ell $. So, the $ \ell $-visible part of the 
output sequence $ \vec{t} $, denoted as $ \proj{\vec{t}}_{\ell}^\Gamma $, is:
\begin{align*}
\proj{\vec{t}}_\ell^\Gamma \defn \configs{ \configs{x, n}~|~\forall \configs{x, 
n} \in \vec{t}.~ \Gamma(x) \LEQ \ell}
\end{align*}
Two memory looks the same to the attacker at $ \ell $:
\begin{align*}
m_1 \loweq_{\ell}^\Gamma m_2 \iff \forall x \in  \Vars. ~\Gamma(x) \LEQ \ell 
\sat m_1(x) = m_2(x)
\end{align*}
The attacker's knowledge in Gradual Release is shown below:
\begin{multline*}
k_{\cod{GR}}(c,m,\vec{t}, \ell, \Gamma) = \{ m' ~|~ m \loweq_{\ell}^\Gamma m' \\
\AND  \configs{c, m'} \xrightarrow{\vec{t_1}} \configs{c',m''} 
\xrightarrow{\vec{t_2}} m'''  \AND \proj{\vec{t_1}}_\ell^\Gamma = 
\proj{\vec{t}}_\ell^\Gamma
\}
\end{multline*}

\begin{Definition}[Gradual Release]
\begin{multline*}
\forall c, m, m', \vec{t}, i. ~~
\configs{c,m} \xrightarrow{\vec{t}}m' \AND 
\\
\vec{t}_{[i]}\not = r  \implies
k_{\cod{PL}}(c,m,\vec{t}_{[:i]}, A) = k_{\cod{PL}}(c,m,\vec{t}_{[:i-1]}, A)
\end{multline*}
\end{Definition}
\begin{proof}
From the semantics of $ \dashrightarrow_A $, we know:
\[
\vec{t}_{[i]}.\lockset \subseteq \lockset_A \iff \vec{t}_{[i]} = l \iff 
\vec{t}_{[i]} \not = r
\]
We can thus rewrite Paralock's security property as follow:
\begin{multline*}
\forall c, m, m', A, \vec{t}, i.~
\configs{c, m, \lockset} \dashrightarrow_A^{\vec{t}} m' \\
\forall \vec{t}_{[i]} \not = r.~~ k_{\cod{PL}}(c, m, \vec{t}_{[:i]}, A) = 
k_{\cod{PL}}(c, m, \vec{t}_{[:i-1]}, A)
\end{multline*}
We note that the subset relation of all locks forms a Denning's 
Lattice $ \Lattice_{\lock} $, that is:
\begin{multline*}
\forall \ell_1, \ell_2\in \Lattice_{\lock}, \lockset_1, \lockset_2.~~
\ell_1 \defn \lockset_1 \AND \ell_2 \defn \lockset_2  \implies \\
\ell_1 \LEQ \ell_2 \iff \lockset_1 \subseteq \lockset_2
\end{multline*}
With $ \Lattice_{\lock} $ and $ \Gamma_A $, we can find $ \ell \in  
\Lattice_{\lock}  $ that $ \ell \defn \lockset_A  $, we know by definition that:
\[
\forall \vec{t}.~~ \proj{\vec{t}}_A = \proj{\vec{t}}_\ell^{\Gamma_A} = 
\configs{\configs{x,n,\lockset}~|~\spec(x,a) 
	\subseteq \lockset_A }  
\]
\[
\forall m_1, m_2. ~~m_1 \loweq_{A} m_2 \iff m_1 \loweq_{\ell}^{\Gamma_A} m_2
\]
\[
\forall c,m, \vec{t}.~~ k_{\cod{PL}}(c, m, \vec{t}, A) = k_{\cod{GR}}(c, m, 
\vec{t}, \ell, \Gamma_A)
\]
Therefore, we know for each attacker $ A = (a, \lockset_A) $ in paralock, its 
policy with semantics $ \dashrightarrow_A $ is equivalent to Gradual Release 
with $ \Gamma_A $ .
\end{proof}

%We construct a security environment $ \Gamma_A $ for each attacker $ A $:
%\[
% \forall x \in \Vars.~~ \Gamma_A(x) = \spec(x,a), \text{ where } A 
% = (a, \lockset_A).
%\]
%For the output events in Paralock, we also categorize them into two groups for 
%each attacker $ A = (a, \lockset_A) $:
%\begin{mathpar}
%\inferrule[Output Event]{ \configs{e,m}\evalto n 
%	\and l = \configs{x, n, \lockset} 
%	\and \lockset \subseteq \lockset_A}
%{\configs{x:=e,m,\lockset} \dashrightarrow^{l}_A \configs{\Skip, 
%		m,\lockset}}
%\and
%\inferrule[Release Output Event]{ \configs{e,m}\evalto n 
%	\and r = \configs{x, n, \lockset}
%	\and \lockset \subseteq \lockset_A}
%{\configs{x:=e,m,\lockset} \dashrightarrow^{r}_A \configs{\Skip, 
%		m,\lockset}}
%\end{mathpar}














==> symbol-table.tex <==
\begin{table*}
\centering
\setlength\extrarowheight{1pt}
\begin{tabular}{lL{15cm}} 
\thline{1} 
\\[-2ex]
\textbf{Notation} & \textbf{Description} 
\\[0.5ex] 
\thline{0.5}
	$ l $ & a security level (domain $ \AllLevels $) \\
	$ L $  & a set of security levels, $ L \subseteq \AllLevels $ \\
   	$ \sentity $ & a security entity (domain $ \mathbb{E} $)\\
   	$ s $ & a security event (domain $ \mathbb{S} $) \\
    $ \lab $ & a security label (domain $ \mathbb{B} $) \\  
    $ e $ & an expression  of the language \\
    $ E $ & a set of expressions  \\
    $ c $ & a command of the language \\
    $ m $ & memory, mapping from variable to integers \\
    $ ch $ & \hl{an output channel}, included in domain $ \mathbb{E} $  \\
    $ n $ & an integer (domain $ \mathbb{N} $)\\
    $ \gamma $ & a state sensitivity \\
 	
 	$ t $ 
 	& an output event, defined as a triple $ \configs{ch, n, \gamma}  $ \\
 	
 	$ \vec{t} $ & a sequence of output event, defined as $ t_0 \cdot t_1 \cdot 
 	... \cdot t_n $. \\
    
    $ \trace $ 
    & a trace of a program, defined as  $ \configs{c_0, m_0} 
    \xrightarrow[]{t_1} \configs{c_1, m_1}  \cdots 
    \xrightarrow[]{t_n}{}  \configs{c_n, m_n} $.\\
    
    
	\\[-2ex]\thline{0.1} \\[-2ex]
	\multicolumn{2}{l}{~~~~~~Functions}\\[0.5ex]
	\thline{0.1}	\\[-2ex]
	
	$ \len{\trace} $ & length of the trace, returning the number of evaluation 
	steps in the trace $ 
	\trace $ \\
	$ \len{\vec{t}} $ & length of the sequence of output events $ \vec{t} $ \\
	
	$ \trace_{[i]} $ & the ending state of the $ i $-th evaluation 
	step in trace $ \trace $, e.g. $ \configs{c_i, m_i} $.\\
	$ \vec{t}_{[i]} $ & the $ i $-th event in the sequence of outputs $ 
	\vec{t}  $, e.g. $ \configs{ch_i, n_i, \gamma_i} $.\\
	
	$ \trace_{\pref i} $ & the prefix sub-trace of trace $ \trace $, starting 
	from the initial state to (included) the ending state  of the $ i $-th 
	evaluation step. 
	\\
	$ \vec{t}_{\pref i} $ & the prefix sub-sequence of outputs $ \vec{t} $ from 
	beginning to (including)  the $ i $-th event.\\
	
	$ \trace_{\suff i} $ & the suffix sub-trace of trace $ \trace $ starting 
	with (included) the ending state of the $ i $-th evaluation step.\\	
    
    $ \psemantics{b}{\trace} $ &interpretation of label $ b $ at the ending 
    state of trace $ \trace $, returning a set of security labels. \\
	
	$ \closure{m}_{E} $ & a memory closure of $ m $ on the set of expression $ 
	E $ (Definition~\ref{def:mclosure}), returning a set of memory.\\
	
	$ \closure{m}_{l, \Gamma} $ & \hl{initial knowledge}\\
	$ \closure{m}_{p} $ & \\
	$ \closure{m}_{\configs{\vec{k},a}} $ & \\
	
	$ \Gamma $ & 
	a security environment, mapping from security entities to its concrete 
	level set \\
	
	$ \Gamma_{\trace} $ & 
	security environment at the ending state of trace \\
	
	$ \proj{\trace} $ & \hl{visibility of the trace $ \trace $, returning a 
	sequence of output events}.  \\
	
	$ \allowence(m) $ & policy allowance, returning a set of memory 
	
	 \\[-2ex]\thline{0.1} \\[-2ex]
	\multicolumn{2}{l}{~~~~~~Relations}\\[0.5ex]
	\thline{0.1}	\\[-2ex]
	
	$ m_1 \loweq_{l}^{\Gamma} m_2  $ & memory equivalence  
	(Definition~\ref{def:mem-eq}) \\
	
	$ \sim  $ & trace indistinguishably \\
	
	$ \equiv  $ & an equivalence relation on two traces \\
	
	$ \trace  \wrap  \configs{c, m, \vec{t}}  $ &  trace $ \trace $ 
	starts with program $ c $ and initial memory $ m $ and generates 
	output sequence $ \vec{t} $ \\
	$ \configs{c, m} \termout \vec{t} $ & there exists a trace which 
	starts with program $ c $ and initial memory $ m $ and generates 
	output event sequence $ \vec{t} $ \\

\thline{1}
\end{tabular}
\caption{List of Symbols}
\end{table*}

==> while-semantics.tex <==
\begin{figure*}
\begin{mathpar}
\inferrule{ }{\configTwo{\Mem}{n} \evalto {n}} 
\and
\inferrule{ }{\configTwo{\Mem}{x} \evalto {\Mem(x)}}
\and
\inferrule{\inferrule{}{\configTwo{\Mem}{e_1} \evalto {n_1} \\\\
	\configTwo{\Mem}{e_2} \evalto {n_2}} \and \
  n = n_1\ \op\ n_2}
 {
  \configTwo{\Mem}{e_1\ \op\ e_2} \evalto {n}}
\end{mathpar}

\begin{mathpar}

\inferrule[S-Assign]
{\configTwo{\Mem}{e} \evalto {n} }
{\configTwo{\Mem}{\assign{x}{e}} \To 
\configTwo{\Mem\Mupdate{x}{n}}{\Skip} }
\and
\inferrule[S-If1]
{\configTwo{\Mem}{e} \evalto n \quad n \neq 0 }
{\configTwo{\Mem}{\ifcmd{e}{\cmd_1}{\cmd_2}} \To 
\configTwo{\Mem}{\cmd_1}}
\and
\inferrule[S-If2]
{\configTwo{\Mem}{e} \evalto n \quad n = 0 }
{\configTwo{\Mem}{\ifcmd{e}{\cmd_1}{\cmd_2}} \To 
\configTwo{\Mem}{\cmd_2}}
\and
\inferrule[S-SecurityOutput]
{\configTwo{\Mem}{e} \evalto {n} }
{\configTwo{\Mem}{\outcmd{\ell}{e}}_{\gamma} \xrightarrow{(\ell,n,\gamma)} 
	\configTwo{\Mem}{\Skip}_{\gamma} }
\and
\inferrule[S-Skip]
{ }{\configTwo{\Mem}{\Skip;\cmd} \To \configTwo{\Mem}{\cmd}}
\and
\inferrule[S-Seq]
{\configTwo{\Mem}{\cmd_1} \xrightarrow{(\ell,n,\gamma)} 
	\configTwo{\Mem'}{\cmd_1'}}
{\configTwo{\Mem}{\cmd_1; \cmd_2} \xrightarrow{(\ell,n,\gamma)}  
	\configTwo{\Mem'}{\cmd_1';\cmd_2}}
\and
\inferrule[S-While]
{ }
{\configTwo{\Mem}{\while{e}{\cmd}} \To 
	\configTwo{\Mem}{\ifcmd{e}{(\cmd;\while{e}{\cmd})}{\Skip}} }
\and
%\inferrule[S-Output]
%{\configTwo{\Mem}{e} \evalto {n} }
%{\configTwo{\Mem}{\outcmd{\ell}{e}} \xrightarrow{(\ell,n)} 
%	\configTwo{\Mem}{\Skip} }
%\and
\\
%\inferrule[S-Source]
%{}
%{\configTwo{\Mem}{\cmd{\ell}{x}} \To
%	\configTwo{\Mem}{\Skip}_{\gamma\Mupdate{x}{\ell}} }
%\and

%\inferrule[S-Update]
%{}
%{\configTwo{\Mem}{\updatecmd{\ell}{x}} \To
%	\configTwo{\Mem}{\Skip}_{\gamma\Mupdate{x}{\ell}} }

\end{mathpar}

% \begin{mathpar}
% \inferrule[S-Seq]
% {\configTwo{\Mem}{\cmd_1} \evalto \Mem' \quad \configTwo{\Mem'}{\cmd_2} \evalto \Mem''}{\configTwo{\Mem}{\cmd_1;\cmd_2} \evalto \Mem''}
% \if 0
%   \and
% \inferrule[S-Seq2]
% {\configTwo{\Mem}{\cmd_1} → \configTwo{\Mem'}{\cmd_1'}}{\configTwo{\Mem}{\cmd_1;\cmd_2} → \configTwo{\Mem'}{\cmd_1';\cmd_2}}
% \fi
%   \and
% \inferrule[S-Assign]
% {\configTwo{e}{\Mem}\evalto n}{\configTwo{\Mem}{x = e} \evalto \Mem\{x \mapsto n\}}
%   \and
% \inferrule[S-If1]
% {\configTwo{e}{\Mem}\evalto 1 \quad \configTwo{\Mem}{\cmd_1} \evalto \Mem'}
% {\configTwo{\Mem}{\ifcmd{e}{\cmd_1}{\cmd_2}} \evalto {\Mem'}}
%   \and
% \inferrule[S-If2]
% {\configTwo{e}{\Mem}\evalto 0 \quad \configTwo{\Mem}{\cmd_2} \evalto \Mem'}
% {\configTwo{\Mem}{\ifcmd{e}{\cmd_1}{\cmd_2}} \evalto {\Mem'}}
%   \and
% \inferrule[S-While1]
% {\configTwo{e}{\Mem}\evalto 1 \quad \configTwo{\Mem}{\cmd;\while{e}{\cmd}} \evalto \Mem'}
% {\configTwo{\Mem}{\while{e}{\cmd}} \evalto {\Mem'}}
%   \and
% \inferrule[S-While2]
% {\configTwo{e}{\Mem}\evalto 0}
% {\configTwo{\Mem}{\while{e}{\cmd}} \evalto {\Mem}}
%
% \end{mathpar}
\caption{Semantics of the Source Language.}
\label{fig:while-semantics}
\end{figure*}


==> while-split.tex <==
\begin{figure*}
\begin{mathpar}
\inferrule{ }{\configTwo{\Mem, \pshot}{n} \evalto {n}} 
\and
\inferrule{ \pshot(x)=\ell }{\configTwo{\Mem, 
\pshot}{x} \evalto {\Mem(x^\ell)}}
\and
\inferrule{\inferrule{}{\configTwo{\Mem,\pshot}{e_1} \evalto {n_1} \\\\
	\configTwo{\Mem,\pshot}{e_2} \evalto {n_2}} \and \
  n = n_1\ \op\ n_2}
 {
  \configTwo{\Mem,\pshot}{e_1\ \op\ e_2} \evalto {n}}
\end{mathpar}

%\begin{mathpar}
%\inferrule{ }{\configTwo{\Mem, \pshot}{\ell} \evalto {\ell}}
%\and
%\inferrule{\configTwo{\Mem, \pshot}{e} \evalto {\True} \\
%	\configTwo{\Mem, \pshot}{p} \evalto {\ell} }
%{\configTwo{\Mem, \pshot}{e?p\circ q} \evalto {\ell}}
%\and
%\inferrule{\configTwo{\Mem, \pshot}{e} \evalto {\False} \\
%	\configTwo{\Mem, \pshot}{q} \evalto {\ell} }
%{\configTwo{\Mem, \pshot}{e?p\circ q} \evalto {\ell}}
%\end{mathpar}

\begin{mathpar}
\inferrule[S-Skip]
{ }{\configTwo{\Mem, \pshot}{\Skip;\cmd} \To 
\configTwo{\Mem,\pshot}{\cmd}}
\and
\inferrule[S-Assign]
{\configTwo{\Mem, \pshot}{e} \evalto {n} \\ 
\pshot(x) =  \ell \\ (\Mem',\pshot') = Update(\penv, s, \Mem, 
\Mem\Mupdate{x^\ell}{n})}
{\configTwo{\Mem, \pshot}{\assign{x}{e}} \To 
	\configTwo{\Mem', \pshot'}{\Skip} 
}
\and
\inferrule[S-Output]
{\configTwo{\Mem, \pshot}{e} \evalto {n} }
{\configTwo{\Mem, \pshot}{\outcmd{\ell}{e}} \xrightarrow{(\ell,n)} 
\configTwo{\Mem, \pshot}{\Skip} }
\and
\inferrule[S-Seq]
{\configTwo{\Mem, \pshot}{\cmd_1} \xrightarrow{(\ell,n)} 
\configTwo{\Mem'}{\cmd_1'} }
{\configTwo{\Mem, \pshot}{\cmd_1; \cmd_2} \xrightarrow{(\ell,n)}  
\configTwo{\Mem', \pshot}{\cmd_1';\cmd_2}}
\and
\inferrule[S-If1]
{\configTwo{\Mem, \pshot}{e} \evalto n \quad n \neq 0 }
{\configTwo{\Mem, \pshot}{\ifcmd{e}{\cmd_1}{\cmd_2}} \To 
\configTwo{\Mem}{\cmd_1}}
\and
\inferrule[S-If2]
{\configTwo{\Mem, \pshot}{e} \evalto n \quad n = 0 }
{\configTwo{\Mem, \pshot}{\ifcmd{e}{\cmd_1}{\cmd_2}} \To 
\configTwo{\Mem}{\cmd_2}}
\and
\inferrule[S-While]
{ }
{\configTwo{\Mem, \pshot}{\while{e}{\cmd}} \To \configTwo{\Mem, 
		\pshot}{\ifcmd{e}{(\cmd;\while{e}{\cmd})}{\Skip}} }
\end{mathpar}

% \begin{mathpar}
% \inferrule[S-Seq]
% {\configTwo{\Mem}{\cmd_1} \evalto \Mem' \quad \configTwo{\Mem'}{\cmd_2} 
%\evalto \Mem''}{\configTwo{\Mem}{\cmd_1;\cmd_2} \evalto \Mem''}
% \if 0
%   \and
% \inferrule[S-Seq2]
% {\configTwo{\Mem}{\cmd_1} → \configTwo{\Mem'}{\cmd_1'}}{\configTwo{\Mem}{\cmd_1;\cmd_2} → \configTwo{\Mem'}{\cmd_1';\cmd_2}}
% \fi
%   \and
% \inferrule[S-Assign]
% {\configTwo{e}{\Mem}\evalto n}{\configTwo{\Mem}{x = e} \evalto \Mem\{x \mapsto n\}}
%   \and
% \inferrule[S-If1]
% {\configTwo{e}{\Mem}\evalto 1 \quad \configTwo{\Mem}{\cmd_1} \evalto \Mem'}
% {\configTwo{\Mem}{\ifcmd{e}{\cmd_1}{\cmd_2}} \evalto {\Mem'}}
%   \and
% \inferrule[S-If2]
% {\configTwo{e}{\Mem}\evalto 0 \quad \configTwo{\Mem}{\cmd_2} \evalto \Mem'}
% {\configTwo{\Mem}{\ifcmd{e}{\cmd_1}{\cmd_2}} \evalto {\Mem'}}
%   \and
% \inferrule[S-While1]
% {\configTwo{e}{\Mem}\evalto 1 \quad \configTwo{\Mem}{\cmd;\while{e}{\cmd}} \evalto \Mem'}
% {\configTwo{\Mem}{\while{e}{\cmd}} \evalto {\Mem'}}
%   \and
% \inferrule[S-While2]
% {\configTwo{e}{\Mem}\evalto 0}
% {\configTwo{\Mem}{\while{e}{\cmd}} \evalto {\Mem}}
%
% \end{mathpar}
\caption{Semantics of the Source Language.}
\label{fig:while-semantics}
\end{figure*}


==> while-typing.tex <==
\begin{figure*}[h]
\begin{mathpar}
\inferrule*[right=T-Const]{ }{ \G  \proves n : \bot }
\and
\inferrule*[right=T-Var]{	\G(x) = \Type}
     {\G  \proves x : \Type}
\and
\inferrule*[right=T-Op]{\G \proves e : \Type_1 \and \G \proves e' : \Type_2}
     {\G \proves e\ \op\ e' : \Type_1\join \Type_2}
 \end{mathpar}
\caption{Typing Rules: Expressions.}
\label{fig:while-typing:exp}
%\begin{mathpar}
%\inferrule*[right=T-Skip]
%{ }{ \G, \pc \proves \Skip   ~|~\G }
%\and
%\inferrule*[right=T-Seq]
%{\G, \pc \proves \cmd_1 ~|~\G'
%	\quad \G', \pc \proves \cmd_2  ~|~\G''}
%{\G, \pc \proves \cmd_1;\cmd_2  ~|~\G''}
%\and
%\inferrule*[right=T-If]
%{ \G \proves e:\Type 
%	\quad\quad  \G, \Type \join \pc \proves \cmd_1 ~|~\G' 
%	 \quad\quad  \G, \Type \join \pc \proves \cmd_2  ~|~\G''}
%{ \G, \pc \proves \ifcmd{e}{\cmd_1}{\cmd_2}  ~|~\G'\join \G'' }
%\\
%\inferrule*[right=T-Assign]
%{ \G \proves e: \Type 
%%	\quad \valid{\hypo(\before{\eta}) \sat \Type \join \pc \absleq \G(x)} \quad 
%%{ \forall v \in \liveset{\actset}(\after \eta).  x \not \in \free(\G(v))}	 
%}
%{  \G, \pc \proves \assigneta{x}{e}   ~|~\G[x \mapsto \Type ]}
%\and
%\inferrule*[right=T-Output]
%{ \G \proves e:\Type 
%	\quad
%	\G, \Type \join \pc \proves e : \Type  
%	\quad
%	\proves \hypo \sat \Type \LEQ \ell}
%{ \G, \pc \proves \outcmd{\ell}{e}  ~|~\G}
%\and
%
%\inferrule*[right=T-While]
%{\G_i \proves e: \Type_i 
%	\quad
%	 \G_i, \Type_i \join \pc \proves \cmd ~|~\G_{i+1}
%	\quad 0\leq i \leq n
%	\quad \G_n = \G_{n+1}}
%{ \G, \pc \proves \while{e}{\cmd} ~|~\G_n }
%\end{mathpar}
\begin{mathpar}
\inferrule*[right=T-Skip]
{ }{ \G, \pc \proves \Skip   }
\and
\inferrule*[right=T-Seq]
{\G, \pc \proves \cmd_1 
	\quad \G, \pc \proves \cmd_2  }
{\G, \pc \proves \cmd_1;\cmd_2 }
\and
\inferrule*[right=T-If]
{ \G \proves e:\Type 
	\quad\quad  \G, \Type \join \pc \proves \cmd_1  
	 \quad\quad  \G, \Type \join \pc \proves \cmd_2 }
{ \G, \pc \proves \ifcmd{e}{\cmd_1}{\cmd_2}   }
\\
\inferrule*[right=T-Assign]
{ \G \proves e: \Type, x: \Type' 
	\quad \tau \LEQ \Type'}
{  \G, \pc \proves \assigneta{x}{e} }
\and
\inferrule*[right=T-Output]
{ \G \proves e:\Type 
	\quad
	\G, \Type \join \pc \proves e : \Type  
	\quad
	\proves \hypo \sat \Type \LEQ \ell}
{ \G, \pc \proves \outcmd{\ell}{e}  }
\and

\inferrule*[right=T-While]
{\G \proves e: \Type
	\quad
	\G, \Type \join \pc \proves \cmd }
{ \G, \pc \proves \while{e}{\cmd}}
\end{mathpar}
\caption{Typing Rules: Commands.}
\label{fig:while-typing:commands}
\end{figure*}

